Tessellated Linear Model for Age Prediction from Voice

Voice biometric tasks, such as age estimation require modeling the often complex relationship between voice features and the biometric variable. While deep learning models can handle such complexity, they typically require large amounts of accurately labeled data to perform well. Such data are often scarce for biometric tasks such as voice-based age prediction. On the other hand, simpler models like linear regression can work with smaller datasets but often fail to generalize to the underlying non-linear patterns present in the data. In this paper we propose the Tessellated Linear Model (TLM), a piecewise linear approach that combines the simplicity of linear models with the capacity of non-linear functions. TLM tessellates the feature space into convex regions and fits a linear model within each region. We optimize the tessellation and the linear models using a hierarchical greedy partitioning. We evaluated TLM on the TIMIT dataset on the task of age prediction from voice, where it outperformed state-of-the-art deep learning models.

==> sections/approach.tex <==


% % \begin{table*}[!ht]
% % \centering
% % \caption{A comparison between TLM and other age estimation models using TIMIT dataset for training and testing}
% % \resizebox{\textwidth}{!}{%
% % \begin{tabular}{lcccl}
% % \hline \vspace{-0.2cm} \\

% % \textbf{Method} & \multicolumn{1}{l}{\textbf{Age RMSE }} & \multicolumn{1}{l}{\textbf{Age MAE}} & \multicolumn{1}{l}{\textbf{Height  RMSE}} & \multicolumn{1}{l}{\textbf{Height MAE}} \\
% % \hline  \vspace{-0.2cm} \\

% % Common sense test         &7.52                 & 5.55                      & 9.06                      & 7.40\\
% % TLM with oracle         &1.18
% %                 & 0.49                  & 1.13                     & 0.34 \\
% % \hline
% % Linear Regression& 5.79   & 4.49             & 6.73            & 5.26 \\ 

% % K-means and Linear Regression    &  7.69           & 5.88 & 8.33           & 6.53  \\ 
% % Random Forest & 6.58    & 4.85             &6.82             & 5.37 \\ 

% % MLP with ReLU & 6.79   & 4.73        & 7.33         & 5.75\\ 
% % % Linear Regression + mixup& 5.77  & 4.48             & 6.78            & 5.28 \\ 

% % % K-means and Linear Regression   + mixup &  6.61          & 5.22 & 7.32           & 5.77 \\ 

% % % Random Forest + mixup & 6.52    & 4.99            & 6.87             & 5.39 \\ 

% % % MLP with ReLU + mixup & -    & -          & -          & -\\ 
% % \hline
% % Singh et al. \cite{singh2016short}          & 8.16                    & 5.83                      & 6.50                       & 5.0 \\
% % NRT \cite{memon2019neural}       &9.13                   &  7.19                    & 16.71                          & 14.31  \\



% % Manav et al. \cite{kaushik2021end}(single-task)   & 7.16               & 5.03                      & 6.69                     &  5.11\\

% % Manav et al. \cite{kaushik2021end} (multi-task)    & 8.07              & 5.63
% %                      & 6.77                    & 5.22 \\

% % Gupta et al.\cite{gupta2022estimation} & 5.86    & 4.13             & 7.01             & 5.41\\ 

% % \hline

% % % TitaNet + TLM   & 5.99             & 4.26          & 6.62             & 5.11 \\ 
% % TitaNet + TLM (Hard routing) &   5.62         & 4.09         & 6.70             & 5.21  \\ 



% % TitaNet + TLM (Soft routing)   &    5.49          & 4.02          & -             & -   \\ 


% % TitaNet + TLM  (Features Optimization)     & \textbf{5.36}             & \textbf{3.97}          & -             & -  \\ \hline
% % % Wav2Vec2 + TLM   &           & -      & -             & - \\ 
% % % Wav2Vec2 + TLM  + mixup &  -      & -        & -             & -   \\ 


% % % Wav2Vec2 + TLM + weighted ensemble   &    -        & -          & -             & -   \\ 


% % % Wav2Vec2 + TLM + Features Optimization     & -             & -           & -             & -  \\ 


% % \hline \hline

% % \end{tabular}
% % }
% % \label{table:age_prediction_comparison}
% % \end{table*}
% % \begin{algorithm}
% % \label{alg:tlm}
% % \caption{Tessellated Linear Model}
% % \begin{algorithmic}[1]
% % \Procedure{BuildTree}{$D_n$}
% % \State Initialize $t_n, \tau_n, \theta_{nl}, \theta_{nr}$
% % \State $\text{best\_reduction} \gets - \infty$
% % \State $\text{best\_threshold} \gets \text{None}$
% % \State $\theta_{n} \gets \text{Regressor}(D_{n}, \theta_{n})$

% % \State $\text{error}_{np} \gets \text{RegressionError}(D_{n}, \theta_{n})$

% % \For{$t_i \in t_n$}
% %     \State $(t_i^*, \tau_n) \gets \text{Classifier}(D_n, t_i, \tau_n)$
% %     \State $D_{nl}, D_{nr} \gets \text{Partition}(D_n, t_i^*)$
% %     \State $\theta_{nl} \gets \text{Regressor}(D_{nl}, \theta_{nl})$
% %     \State $\theta_{nr} \gets \text{Regressor}(D_{nr}, \theta_{nr})$
% %     \State $\text{error}_{nl} \gets \text{RegressionError}(D_{nl}, \theta_{nl})$
% %     \State $\text{error}_{nr} \gets \text{RegressionError}(D_{nr}, \theta_{nr})$
% %     \State $\text{total\_reduction} \gets \text{error}_{np} - \text{error}_{nl} + \text{error}_{nr}$
% %     \If{$\text{total\_reduction} > \text{best\_reduction}$}
% %         \State $\text{best\_reduction} \gets \text{total\_reduction}$
% %         \State $\text{best\_threshold} \gets t_i^*$
% %     \EndIf
% % \EndFor
% % \State $t_n^* \gets \text{best\_threshold}$
% % \State $D_{nl}, D_{nr} \gets \text{Partition}(D_n, t_n^*)$
% % \For{$D_n \in \{D_{nl}, D_{nr}\}$}
% %     \If{$D_n$ is pure}
% %         \State \textbf{continue}
% %     \Else
% %         \State \textsc{BuildTree}($D_n$)
% %     \EndIf
% % \EndProcedure


% % \end{algorithmic}

% % \end{algorithm}


% \begin{algorithm}
% \caption{Tessellated Linear Model}
% \label{alg:TLM}  % Label for reference
% \begin{algorithmic}[1]
% \Procedure{BuildTree}{$D_n$}
% \State Initialize $t_n, \tau_n, \theta_{nl}, \theta_{nr}$
% \State $\text{best\_reduction} \gets -\infty$
% \State $\text{best\_threshold} \gets \text{None}$
% \State $\theta_{n} \gets \text{Regressor}(D_{n}, \theta_{n})$
% \State $\text{error}_{np} \gets \text{RegressionError}(D_{n}, \theta_{n})$
% \For{$t_i \in t_n$}
%     \State $(t_i^*, \tau_n) \gets \text{Classifier}(D_n, t_i, \tau_n)$
%     \State $D_{nl}, D_{nr} \gets \text{Partition}(D_n, t_i^*)$
%     \State $\theta_{nl} \gets \text{Regressor}(D_{nl}, \theta_{nl})$
%     \State $\theta_{nr} \gets \text{Regressor}(D_{nr}, \theta_{nr})$
%     \State $\text{error}_{nl} \gets \text{RegressionError}(D_{nl}, \theta_{nl})$
%     \State $\text{error}_{nr} \gets \text{RegressionError}(D_{nr}, \theta_{nr})$
%     \State $\text{total\_reduction} \gets \text{error}_{np} - \text{error}_{nl} + \text{error}_{nr}$
%     \If{$\text{total\_reduction} > \text{best\_reduction}$}
%         \State $\text{best\_reduction} \gets \text{total\_reduction}$
%         \State $\text{best\_threshold} \gets t_i^*$
%     \EndIf
% \EndFor
% \State $t_n^* \gets \text{best\_threshold}$
% \State $D_{nl}, D_{nr} \gets \text{Partition}(D_n, t_n^*)$
% \For{$D_n \in \{D_{nl}, D_{nr}\}$}
%     \If{$D_n$ is pure}
%         \State \textbf{continue}
%     \Else
%         \State \textsc{BuildTree}($D_n$)
%     \EndIf
% \EndFor
% \EndProcedure
% \end{algorithmic}
% \end{algorithm}

% \section{Tessellated Linear Model}
% \label{sec:approach}



% In this section, we will describe the Tessellated Linear Model (TLM) for the regression task, which aims to partition the input space and fit separate linear models in each region. We optimize both the tessellation and the regression functions using a recursive binary splitting approach.


% Let the input space $\mathcal{X} \subset \mathbb{R}^d$ and the response variable $y \in \mathbb{R}$. The goal of the TLM is to partition $\mathcal{X}$ into convex cells where each cell can be modeled by a simple linear function. We define the tessellation $\tau$ as a partition of $\mathcal{X}$ into $N$ disjoint convex cells:
% \[
% \tau(\mathcal{X}) = \{C_1, \dots, C_N\}
% \]
% satisfying $\bigcup_{n=1}^{N} C_n = \mathcal{X}$, and each $C_n$ is a convex subset of $\mathcal{X}$. 



% Within each region $C_n$, we fit a linear regression function $r_{\theta_{n}}$ to approximate the response $y$. The linear model for a point $\mathbf{x} \in C_n$ is given by:
% \[
% \hat{y}(\mathbf{x}) =r_{\theta_{n}}^\top \mathbf{x} + b_n
% \]
% where $r_{\theta_{n}} \in \mathbb{R}^d$ is the regression coefficient vector, and $b_n \in \mathbb{R}$ is the bias term for region $C_n$.


% The tessellation process $\tau$ is optimized recursively by scanning potential binary boundaries based on the response variable $y$. At each step, a classifier $h_\theta$ is trained to split the data into two regions: left ($y \leq t$) and right ($y > t$), where $t$ is the threshold that defines the boundary. The classifier $h_\theta$ assigns each point $\mathbf{x} \in \mathcal{X}$ to either the left or right region:
% \[
% h_\theta(\mathbf{x}) = 
% \begin{cases} 
% 1 & \text{if } y(\mathbf{x}) \leq t \\
% 0 & \text{if } y(\mathbf{x}) > t
% \end{cases}
% \]

% Once the data is split, separate linear models $r_{\theta_{\text{left}}}$ and $r_{\theta_{\text{right}}}$ are trained on the left and right subsets, respectively. The threshold $t$ is chosen to maximize the reduction in prediction error, defined as the difference between the parent node's regression error and the sum of squared residuals (SSR) for both the left and right regions:

% \begin{align*}
% t^* = \arg\max_t \Bigg( & \text{SSR}_{\text{parent}} - \Bigg( 
%     \sum_{\mathbf{x} \in \text{left}} (y - \hat{y}_{\text{left}}(\mathbf{x}))^2 \\
%     & + \sum_{\mathbf{x} \in \text{right}} (y - \hat{y}_{\text{right}}(\mathbf{x}))^2 \Bigg) \Bigg)
% \end{align*}


% Initially, the parent node's regression model $r_{\theta_{\text{parent}}}$ is trained on the entire dataset.
% The splitting process is repeated recursively, with new classifiers $h_\theta$ and regression models $\theta_n$ trained at each stage, until a stopping criterion is met. The recursion stops when a maximum depth $D$ is reached, or when no further meaningful splits can be made.

% The final prediction for an input $\mathbf{x}$ is made by passing it through a series of classifiers in a hierarchical tree structure. At each node in the tree, a classifier $h_\theta$ guides $\mathbf{x}$ to either the left or right child node, depending on the learned decision boundary at that level. This process is repeated recursively until $\mathbf{x}$ reaches a leaf node, corresponding to a specific region $C_n$. Once $\mathbf{x}$ is assigned to the correct region, the corresponding regression model $r_{\theta_n}$ is used to make the final prediction. Formally, the prediction is given by:

% \[
% \hat{y}(\mathbf{x}) = r_{\theta_{\tau(\mathbf{x})}}^\top \mathbf{x} + b_{\tau(\mathbf{x})}
% \]

% where $\tau(\mathbf{x})$ represents the tessellation procedure to reach node (or region) $C_n$, and $r_{\theta_{\tau(\mathbf{x})}}$ and $b_{\tau(\mathbf{x})}$ are the parameters of the linear model for that region.



\begin{small}
\begin{algorithm}
\fontsize{8}{10}\selectfont

\caption{Tessellated Linear Model}
\label{alg:TLM}  % Label for reference
\begin{algorithmic}
\Procedure{BuildTree}{${D_n}$}
\State Initialize $t_n, \tau_n, \theta_{nl}, \theta_{nr}$
\State $\text{best\_reduction} \gets -\infty$
\State $\text{best\_threshold} \gets \text{None}$
\State $\theta_n \gets \text{Regressor}(D_n, \theta_n)$
\State $\text{error}_{np} \gets \text{RegressionError}(D_n, \theta_n)$
\For{$t_i \in t_n$}
    \State $(t_i^*, \tau_n) \gets \text{Classifier}(D_n, t_i, \tau_n)$
    \State $D_{nl}, D_{nr} \gets \text{Partition}(D_n, t_i^*)$
    \State $\theta_{nl} \gets \text{Regressor}(D_{nl}, \theta_{nl})$
    \State $\theta_{nr} \gets \text{Regressor}(D_{nr}, \theta_{nr})$
    \State $\text{error}_{nl} \gets \text{RegressionError}(D_{nl}, \theta_{nl})$
    \State $\text{error}_{nr} \gets \text{RegressionError}(D_{nr}, \theta_{nr})$
    \State $\text{total\_reduction} \gets \text{error}_{np} - \text{error}_{nl} + \text{error}_{nr}$
    \If{$\text{total\_reduction} > \text{best\_reduction}$}
        \State $\text{best\_reduction} \gets \text{total\_reduction}$
        \State $\text{best\_threshold} \gets t_i^*$
    \EndIf
\EndFor
\State $t_n^* \gets \text{best\_threshold}$
\State $D_{nl}, D_{nr} \gets \text{Partition}(D_n, t_n^*)$
\For{$D_n \in \{D_{nl}, D_{nr}\}$}
    \If{$D_n$ is pure}
        \State \textbf{continue}
    \Else
        \State \textsc{BuildTree}($D_n$)
    \EndIf
\EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm} 
\end{small}



\section{Tessellated Linear Model}
\label{sec:approach}

% [[

% The TLM tessellates the space into a convex cover (of disjoint convex sets), and applies a linear model within each cell. (While 
% piecewise linear models do not require convex cells, non-convex cells make the model considerably more complex to estimate [CITE]).  In the case of a convex cover, the individual cells must be polytopes [CITE]. Thus, the tessellation may be parameterized through the set of linear partitions between cells.

% The TLM itself is {T, L}, where T is the set of linear partitions, and L are the linear predictors.

% The TLM is optimized as  argmin_{T,L} Loss()

% When the features aer themselves optimizable, then the TLM may be described as {T, L, F}.
% optimization is argmin_{TLF} Loss()

% ]]

Given a dataset $\{(\mathbf{x}_i, y_i)\}_{i=1}^N$, where $\mathbf{x}_i \in \mathcal{X} \subset \mathbb{R}^d$ is a feature vector and $y_i \in \mathbb{R}$ is the response variable, our goal is to tessellate the input space $\mathcal{X}$ into disjoint convex regions that are easy to estimate \cite{boyd2004convex} and fit a simple linear model in each region. Formally, let the tessellation $\tau$ represent the partitioning of $\mathcal{X}$ into $N$ disjoint convex regions, known as polytopes \cite{gruber2007convex}:
\[
\tau(\mathcal{X}) = \{C_1, C_2, \dots, C_N\}, \quad \text{where } C_n \subseteq \mathcal{X} \text{ is convex}.
\]

Within each region $C_n$, the relationship between the input $\mathbf{x} \in C_n$ and the response variable $y$ is modeled by a linear regression function:
\[
\hat{y}(\mathbf{x}) = L_{\theta_n}^\top \mathbf{x} + b_n,
\]
where $L_{\theta_n} \in \mathbb{R}^d$ is the regression coefficient vector, and $b_n \in \mathbb{R}$ is the bias term for region $C_n$. 

Our goal is to find both the optimal tessellation $\tau$ and the linear models $L_{\theta_n}$ for each region $C_n$ to minimize the overall prediction error. This can be expressed as minimizing the sum of squared residuals across all regions:
\[
\min_{\tau, L_{\theta_n}} \sum_{n=1}^N \sum_{\mathbf{x} \in C_n} (y - \hat{y}(\mathbf{x}))^2.
\]

The joint optimization of the tessellation and the linear models is a combinatorial problem and is NP-hard. To make this problem tractable, we adopt a greedy approach that iteratively learns a linear predictor to split the space based on the response variable $y$. We scan potential boundaries that minimize the squared error.

At each iteration, we seek to split the input space into two regions using a binary linear predictor. The split is defined by a threshold $t$ on the response variable $y$. Formally, at each step, we define a classifier $h_\theta$ that divides the data into left ($y \leq t$) and right ($y > t$) regions:
\[
h_\theta(\mathbf{x}) = 
\begin{cases} 
1 & \text{if } y(\mathbf{x}) \leq t \\
0 & \text{if } y(\mathbf{x}) > t
\end{cases}
\]
This linear predictor scans for the best boundary $t$ by evaluating the reduction in the prediction error caused by splitting the data. The goal is to minimize the sum of squared residuals (SSR) for the resulting left and right regions, given the linear models fitted to each region:

% \[
% \{t^*, L_{\theta_{\text{left}}}, L_{\theta_{\text{right}}}, h_{\theta}\} = \arg\max_{t, L_{\theta}, h_{\theta}} \Bigg( \text{SSR}_{\text{parent}} - \Bigg( 
%     \sum_{\mathbf{x} \in \text{left}} (y - \hat{y}_{\text{left}}(\mathbf{x}))^2 
%     + \sum_{\mathbf{x} \in \text{right}} (y - \hat{y}_{\text{right}}(\mathbf{x}))^2 
%     \Bigg) \Bigg).
% \]
% \{t^*, L_{\theta_{\text{left}}}, L_{\theta_{\text{right}}}, h_{\theta}\} =
\begin{align*}
 \arg\max_{t, L_{\theta}, h_{\theta}} \Bigg( & \text{SSR}_{\text{parent}} - \Bigg( 
    \sum_{\mathbf{x} \in \text{left}} (y - \hat{y}_{\text{left}}(\mathbf{x}))^2 \\
    & + \sum_{\mathbf{x} \in \text{right}} (y - \hat{y}_{\text{right}}(\mathbf{x}))^2 \Bigg) \Bigg)
\end{align*}



What sets our approach apart from other RvC variations is that we optimize the feature space to enhance the decision boundaries learned by the model. To formally integrate feature optimization into the tessellation process, let $F_{\theta_n}^\top$ be a parametric model that projects the input $\mathbf{X}$ into a new feature space $\mathbf{Z}$. The linear predictor $L_{\theta_n}$ then operates in this transformed space, learning boundaries and fitting linear regression models on the projected features. This transforms the optimization problem as follows:

% \[
% \{t^*, L_{\theta_{\text{left}}}, L_{\theta_{\text{right}}}, F_{\theta}, h_{\theta} \} = \arg\max_{t, L_{\theta}, F_{\theta}, h_{\theta}} \Bigg( \text{SSR}_{\text{parent}} - \Bigg( 
%     \sum_{\mathbf{x} \in \text{left}} (y - \hat{y}_{\text{left}}(\mathbf{x}))^2 + 
%     \sum_{\mathbf{x} \in \text{right}} (y - \hat{y}_{\text{right}}(\mathbf{x}))^2 \Bigg) \Bigg).
% \]
% \{t^*, L_{\theta_{\text{left}}}, L_{\theta_{\text{right}}}, F_{\theta}, h_{\theta} \} = 
\small
\begin{align*}
\arg\max_{t, L_{\theta}, F_{\theta}, h_{\theta}} \Bigg( & \text{SSR}_{\text{parent}} - \Bigg( 
    \sum_{\mathbf{x} \in \text{left}} (y - \hat{y}_{\text{left}}(\mathbf{x}))^2 \\
    & + \sum_{\mathbf{x} \in \text{right}} (y - \hat{y}_{\text{right}}(\mathbf{x}))^2 \Bigg) \Bigg)
\end{align*}
\normalsize

The final prediction for an input $\mathbf{x}$ is made by passing it through a series of classifiers in a hierarchical tree structure. At each node in the tree, a classifier $h_\theta$ guides $\mathbf{x}$ to either the left or right child node, depending on the learned decision boundary at that level. This process is repeated recursively until $\mathbf{x}$ reaches a leaf node, corresponding to a specific region $C_n$. Once $\mathbf{x}$ is assigned to the correct region, the corresponding regression model $r_{\theta_n}$ is used to make the final prediction. Formally, the prediction is given by:

\[
\hat{y}(\mathbf{x}) = r_{\theta_{\tau(\mathbf{x})}}^\top \mathbf{x} + b_{\tau(\mathbf{x})}
\]

where $\tau(\mathbf{x})$ represents the tessellation procedure to reach node (or region) $C_n$, and $r_{\theta_{\tau(\mathbf{x})}}$ and $b_{\tau(\mathbf{x})}$ are the parameters of the linear model for that region.



==> sections/background.tex <==
\section{Related Work}
\label{sec:related_work}

\subsection{Piece-wise Linear Models}



% Piece-wise linear problems involve functions that can be approximated using multiple linear models, each applicable to a specific region or interval. These problems require the joint optimization of partition boundaries and local linear models, which is a combinatorial probelm that is difficult to optimize. Many existing methods rely on simplifying assumptions about the space, which often result in suboptimal solutions.

% Segmented linear model with binary segmentation  \cite{edwards1965method}


% One of the algorithms used to address such problems is the segmented linear model \cite{hawkins1976point}. This approach splits features into segments based on a change-point detection algorithm and then fits a linear model to each segment. A significant challenge with this approach is determining the optimal change points or partition boundaries. Classical approaches, such as Davies' test \cite{davies1987hypothesis}, assume that the change points are fixed, continuous, and occur consecutively within the space. Another method,  Pruned Exact Linear Time (PELT) \cite{ verzelen2023optimal}, iteratively minimizes a cost function with a penalty term to identify change points. However, PELT is sensitive to the choice of penalty and the cost function. 

% Kernel methods transform the input space into a higher-dimensional space where it becomes linearly separable \cite{cortes1995support, chan2023plame}; however, this approach can be computationally expensive, especially for high-dimensional data. Decision trees, which partition the space based on input features \cite{loh2011classification}, also face difficulties in identifying optimal change points. Neural networks with ReLU activations are capable of approximating piecewise linear functions but typically require large amounts of data and strong regularization. Additionally, these networks assume the continuity of the piecewise linear function, which results in strict boundaries. 


% An example of RvC is the Neural Regression Tree (NRT) \cite{memon2019neural}, which partitions a continuous response variable into discrete categories by creating intervals on the real number line. The categorization process at each node involves a neural classifier that decides how to split the data based on a threshold, which is initially set randomly and then optimized using a "triviality loss" metric—a measure of the squared error between the threshold and the response variable's median. Each node in the NRT is optimized to minimize both classification and threshold errors until the tree reaches a predetermined depth. During inference, the NRT model predicts the interval to which each input belongs and assigns a continuous value by applying a regression rule that simply computes the mean of values within that interval.


Piecewise linear problems involve approximating a complex function by using multiple linear models, each valid within a specific region or interval of the input space. These problems require the joint optimization of both partition boundaries and local linear models, which creates a challenging combinatorial optimization problem. Many existing approaches simplify the problem space by making assumptions, but these often lead to suboptimal solutions. One widely-used method to tackle piecewise linear problems is the segmented linear model \cite{hawkins1976point}. This approach divides the input space into segments based on change-point detection algorithms and fits a linear model to each segment. A key challenge with segmented linear models lies in identifying the optimal change points or partition boundaries. Classical methods, such as Davies' test \cite{davies1987hypothesis}, assume fixed, continuous change points that occur consecutively within the space, limiting flexibility. Another notable algorithm, Pruned Exact Linear Time (PELT) \cite{verzelen2023optimal}, minimizes a cost function for the total segmentation error across all segments, combined with a penalty term, to identify change points. However, PELT is sensitive to the choice of both the penalty value and the cost function.

Another approach for segmented linear models involves their use with binary segmentation \cite{edwards1965method}. Binary segmentation recursively divides the input space into two regions and continues to do so until no additional change points can be detected. This method bears similarities to Regression-via-Classification (RvC) techniques, where classifiers are employed to identify change points and discretize the continuous output into predefined categories. Each category corresponds to a specific range of the target variable. An example of an RvC method is the Neural Regression Tree (NRT) \cite{memon2019neural}, which partitions a continuous response variable into discrete intervals by setting thresholds along the real number line. At each node, a neural classifier determines how to split the data, starting with a randomly initialized threshold. This threshold is then optimized using a "triviality loss" metric, which minimizes the squared error between the threshold and the median of the response variable. During inference, the NRT predicts which interval an input belongs to and applies a simple regression rule, assigning the mean value of the response variable within that interval.



Other methods for piecewise linear problems include kernel methods, which transform the input space into a higher-dimensional space where it becomes linearly separable \cite{cortes1995support, chan2023plame}. While effective, kernel methods can be computationally expensive, particularly for high-dimensional data. Decision trees \cite{loh2011classification}, which partition the space based on input features, also face challenges in identifying optimal change points. Similarly, neural networks with ReLU activations \cite{nair2010rectified} can approximate piecewise linear functions but often require large amounts of data and strong regularization. Moreover, they assume the continuity of the piecewise linear function, which imposes strict boundaries between segments.

The closest approaches to our proposed method are the segmented linear model with binary segmentation and the NRT algorithm. The former uses squared differences in the feature space to segment the data, while the latter employs a classifier with a set of thresholds (such as the median within each segment in NRT) to tessellate the space. However, to the best of our knowledge, no prior work has explored scanning for optimal thresholds based on the response variable and using the reduction in error at each level as a guide for tessellation—especially in the context of voice biometrics tasks.

Our proposed method, the Tessellated Linear Model (TLM), addresses this gap by partitioning the input space into convex regions and applying local linear regressors within each region. This approach allows for more flexible and accurate modeling of non-linear relationships, while maintaining the simplicity and interpretability of linear models.



\subsection{Age Estimation}




Human voices undergo significant changes over time due to physiological factors, such as alterations in the vocal cords, muscles, and lung capacity. This makes age estimation from voice a plausible task in speech processing and biometrics. However, the inherent variability in speech—affected by factors such as health, emotional state, and individual differences in vocal anatomy—presents a substantial challenge. As a result, while age estimates may not always be precise, they are often accurate within a range of values, typically expressed as a confidence interval \cite{singh2019profiling}.

Traditional age estimation methods relied on basic algorithms like Gaussian Mixture Models (GMMs) paired with signal analysis.  One such approach \cite{singh2016short} employed shorter analysis windows (1ms to 4ms) to focus on speech segments during glottal opening, in contrast to the conventional 25ms windows. These shorter windows were believed to better capture subglottal structures, potentially providing more accurate physiometric information from the voice. Additionally, research has explored the combination of short-term cepstral features, like Mel-Frequency Cepstral Coefficients (MFCCs), with utterance-based pitch information to enhance age estimation accuracy \cite{muller2007combining}. Other approaches, such as those proposed by \cite{li2013automatic}, incorporated prosodic features—such as pitch, energy, duration, and formants—alongside acoustic information to model age-related changes in speech.

Recently, the field has shifted towards leveraging deep learning features for more effective age estimation \cite{kaushik2021end, kwasny2020joint, rajaa2021learning, gupta2022estimation}. Approaches such as x-vectors \cite{snyder2017deep, snyder2018x, wan2018generalized}, originally developed for speaker verification and identification, along with features extracted from self-supervised models like Wav2Vec \cite{schneider2019wav2vec} and WavLM \cite{chen2022wavlm}, have gained prominence. These deep learning-based representations outperform traditional handcrafted features by learning directly from the entire speech signal, providing more robust and generalizable solutions. In our experiments, we employ TitaNet \cite{koluguri2022titanet} and WavLM features in conjunction with our proposed Tessellated Linear Model (TLM).



% \begin{figure}[htbp]
%   \centerline{\includegraphics[width=\linewidth,height=0.2\textheight]{figures/tlm_syn.png}}


  
%   \caption{Left: A convex tessellation of the input space. An optimal TLM would determine both the tessellation and the linear estimator parameters within each cell, for optimal prediction. Right: Our hierarchical solution. The space is recursively partitioned in a binary manner for optimal tessellation. Here, the red line shows the first level partition, blue lines show the second level, and green lines show the third level.}
%   \label{fig}
% \end{figure}



\begin{figure}[htbp]
  \centerline{\includegraphics[width=\linewidth,height=0.3\textheight]{figures/tlm_real_depths.png}}


  
  \caption{TLM}
  \label{fig:tlm_real_depths}
\end{figure}




\begin{figure}[htbp]
  \centerline{\includegraphics[width=\linewidth,height=0.3\textheight]{figures/tlm_tree.png}}


  
  \caption{TLM}
  \label{fig:tlm_tree}
\end{figure}




==> sections/experiment_setup.tex <==

\begin{table}[!ht]
\centering
\caption{A comparison between TLM and other age estimation models using TIMIT dataset for training and testing}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcc}
\hline \vspace{-0.2cm} \\

\textbf{Method} & \multicolumn{1}{l}{\textbf{Age RMSE}} & \multicolumn{1}{l}{\textbf{Age MAE}} \\
\hline  \vspace{-0.2cm} \\

Common sense test         &7.52                 & 5.55 \\
TLM with oracle         &1.18                 & 0.49 \\
\hline
Linear Regression& 5.79   & 4.49 \\ 

K-means and Linear Regression    &  7.69           & 5.88 \\ 
Random Forest & 6.58    & 4.85 \\ 

MLP with ReLU & 6.79   & 4.73 \\ 
% Linear Regression + mixup& 5.77  & 4.48 \\ 

% K-means and Linear Regression   + mixup &  6.61          & 5.22 \\ 

% Random Forest + mixup & 6.52    & 4.99 \\ 

% MLP with ReLU + mixup & -    & - \\ 
\hline
Singh et al. \cite{singh2016short}          & 8.16                    & 5.83 \\
NRT \cite{memon2019neural}       &9.13                   &  7.19 \\

Manav et al. \cite{kaushik2021end}(single-task)   & 7.16               & 5.03 \\

Manav et al. \cite{kaushik2021end} (multi-task)    & 8.07              & 5.63 \\

Gupta et al.\cite{gupta2022estimation} & 5.86    & 4.13 \\ 

\hline

TitaNet + TLM (Hard routing) &   5.62         & 4.09 \\ 

TitaNet + TLM (Soft routing)   &    5.49          & 4.02 \\ 

TitaNet + TLM  (Features Optimization)     & \textbf{5.36}             & \textbf{3.97} \\ 
\hline \hline

\end{tabular}
}
\label{table:age_prediction_comparison}
\end{table}
\section{Experimental Setup}
\label{sec:experiment}


\subsection{Data}
For our experiments, we utilized the TIMIT dataset to perform age prediction regression task. The TIMIT dataset consists of 4,610 samples—3,260 from male speakers and 1,350 from female speakers. The test set contains 1,680 samples—1,120 from male speakers and 560 from female speakers. The age distribution of the speakers ranges from 20 to 58 years.

\subsection{TLM }
% \paragraph{Training Process}
We trained the Tessellated Linear Model (TLM) using 192-dimensional embeddings from the Titanet-Large model \cite{koluguri2022titanet}. To construct the tree, we employed logistic regression for data splitting and linear regression for age prediction. At each node, we scanned possible thresholds and trained a classifier to split the data. The split data was then used to train two regression models, and we applied a modified version of mixup \cite{zhang2017mixup} by mixing samples with similar age values. We selected the threshold and models that minimized the total squared error. This process was repeated recursively for each branch until the maximum tree depth was reached or further splitting was no longer meaningful. The TLM training procedure is detailed in Algorithm \ref{alg:TLM}.


% \paragraph{Feature Optimization}
After constructing the tree, we optimized the Titanet embeddings with two residual blocks, each consisting of two fully connected layers with ReLU and Leaky ReLU activations (dropout: 0.2). The optimized features were used to predict age with the TLM. The overall loss was the average of all classifiers (Binary Cross-Entropy) and regressors (Mean Squared Error) losses.


% After constructing the tree, we optimized the Titanet embeddings using two residual blocks. Each residual block \cite{he2016deep} consisted of two fully connected layers with ReLU and Leaky ReLU activations (with a dropout probability of 0.2). The optimized features were then used to predict age using the TLM. The overall loss was calculated as the average of the classifiers and regressors losses. For the classifier, we used Binary Cross-Entropy (BCE) loss, and for the regression tasks, we used Mean Squared Error (MSE) loss.


% \paragraph{Inference Strategies}
We designed two strategies for inference: \textbf{Hard Routing}: The classifier at each node routes the input to a leaf, where the associated linear regression model predicts the response value. \textbf{Soft Routing}: Instead of strict routing, linear regression models at all nodes predict the response. Each node's classifier probability determines its contribution to the final prediction, with the final result being the weighted sum of predictions from all nodes.




% \subsection{Baseline Models}
We compared the performance of TLM with several baseline models that have similar structures, including a MLP with ReLU activation, K-Means with Linear Regression (where we performed K-Means clustering on the data with $k = 10$, matching the number of regions in TLM, and trained a linear regression model for each cluster), Random Forest, and simple Linear Regression. In addition, we compared TLM against three models for age prediction models that was explained in section \ref{sec:related_work}.

% : \cite{singh2016short}, which extracts spectral features using short windows (1ms to 4ms) and uses a random forest for prediction (holding the current state-of-the-art results for height prediction), \cite{kaushik2021end}, an end-to-end deep learning model that combines LSTM and attention mechanisms to predict the target variables, and \cite{gupta2022estimation}, which leverages wav2vec 2.0 embeddings and employs separate transformer encoders for male and female speakers to predict age and height.


\begin{figure}[htbp]
  \centerline{\includegraphics[width=1.0\linewidth]{figures/tlm_tree.png}}


  \captionsetup{font=small}
  \caption{The tree shows the training and test MAE at each node of the TLM model. It illustrates the stepwise reduction in MAE with distinct thresholds defining the regions. Each parent node represents a binary decision based on a chosen threshold, and the MAE is evaluated only on the data samples routed to the region based on the threshold. It is evident that the error is lower for younger speakers, which corresponds to a higher number of training samples in these regions. }
  \label{fig:tlm_tree}
\end{figure}

==> sections/intro.tex <==
\section{Introduction}
\label{sec:intro}

% Regression-via-Classification (RvC) is a technique that transforms the task of predicting a continuous variable into a classification problem, by discretizing the output into predefined categories, each representing a specific range or segment of the continuous outcome. The Neural Regression Tree (NRT) model is an example of RvC. This model partitions a continuous response variable into discrete categories, each represented by intervals on the real number line. The categorization process at each node involves a neural classifier that decides data splits based on a threshold, which are  randomly set within the continuous response range and later optimized using triviality loss, a metric that measures the squared error between the threshold and the response variable median. Each node in the NRT is optimized to minimize both classification and threshold errors.


% Each node in the tree is optimized to simultaneously minimize classification and threshold errors. This optimization continues until the tree achieves a predetermined depth. During the inference phase, the Neural Regression Tree (NRT) model categorizes input features by predicting the interval to which each input belongs. It then assigns a continuous value based on the regression rule associated with that interval. In the NRT model, this regression rule involves simply calculating the mean of the values within the interval.


% While the NRT model offers a promising approach, its focus on classification error and simple regression rules can limit its performance for regression tasks. The model’s focus on joint threshold optimization with the binary classifier restricts it to thresholds close to the median, potentially overlooking more optimal thresholds that minimize regression error. Additionally, the simplicity of the regression rule—using only the mean—might not yield the lowest possible regression error.

% To address these issues, we propose an enhanced NRT framework that scans all possible thresholds rather than focusing solely on median-based metrics. This method allows for a broader exploration of potential decision boundaries. Furthermore, it selects the optimal threshold based on the greatest reduction in regression error. In our revised model, an expert linear regression model is trained for each interval. Our revised framework aims to learn a piecewise linear predictor over linear tessellations of the space —achieved by the classifiers—the combination is jointly optimized. 







% Piecewise linear problems involve functions that can be approximated using multiple linear models, each applicable to a specific region or interval. These problems require the joint optimization of partition boundaries and local linear models, which is a combinatorial probelm that is difficult to optimize. Many existing methods rely on simplifying assumptions about the space, which often result in suboptimal solutions.

% One of the algorithms used to address such problems is the segmented linear model \cite{hawkins1976point}. This approach splits features into segments based on a change-point detection algorithm and then fits a linear model to each segment. A significant challenge with this approach is determining the optimal change points or partition boundaries. Classical approaches, such as Davies' test \cite{davies1987hypothesis}, assume that the change points are fixed, continuous, and occur consecutively within the space. Another method,  Pruned Exact Linear Time (PELT) \cite{ verzelen2023optimal}, iteratively minimizes a cost function with a penalty term to identify change points. However, PELT is sensitive to the choice of penalty and the cost function. 

% Kernel methods transform the input space into a higher-dimensional space where it becomes linearly separable \cite{cortes1995support, chan2023plame}; however, this approach can be computationally expensive, especially for high-dimensional data. Decision trees, which partition the space based on input features \cite{loh2011classification}, also face difficulties in identifying optimal change points. Neural networks with ReLU activations are capable of approximating piecewise linear functions but typically require large amounts of data and strong regularization. Additionally, these networks assume the continuity of the piecewise linear function, which results in strict boundaries. 



% Regression-via-Classification (RvC) \cite{torgo1997regression, memon2019neural, zhao2021hierarchical} is a technique that finds change points using a classifier to discretize the output into predefined categories, each representing a specific range or segment of the continuous outcome. The Neural Regression Tree (NRT) \cite{memon2019neural} model is an example of RvC. This model partitions a continuous response variable into discrete categories, each represented by intervals on the real number line. The categorization process at each node involves a neural classifier that decides data splits based on a threshold, which is randomly set within the continuous response range and later optimized using triviality loss, a metric that measures the squared error between the threshold and the response variable median. Each node in the NRT is optimized to minimize both classification and threshold errors. This optimization continues until the tree reaches a predetermined depth. During the inference phase, the NRT model categorizes input features by predicting the interval to which each input belongs and then assigns a continuous value based on the regression rule associated with that interval. In the NRT model, this regression rule involves simply calculating the mean of the values within the interval.

% We propose a Tessellated Linear Model that determines change points based on the response variable  and greedily tessellates the space using binary classifiers that minimize the regressor's errors. This algorithm belongs to the RvC family. Our framework aims to learn an optimal piecewise linear predictor over linear tessellations of the input space, jointly optimizing the tessellation (achieved by the node classifiers) and the expert linear regression models. By scanning for the best thresholds using the response variable and learning binary classifiers to tessellate the space accordingly, we transform the difficult combinatorial optimization problem into a more tractable learning problem.








% The key contributions of this paper are:

% \begin{enumerate}
%     \item A simplified model for piecewise linear functions that uses linear regression and logistic regression classifiers to tessellate the space and fit a linear model in each segment.
%     \item A comparison of different training and inference strategies.
%     \item Evaluation on two regression tasks from voice data: age prediction and height prediction.
%     \item An evaluation benchmark for age prediction based on Queen Elizabeth II's recordings from 1953 to 2021.
% \end{enumerate}

% In the following sections, we formally describe the Tessellated Linear Model, present experimental results, and discuss the implications of this approach for regression problems in various domains.




% \begin{figure}[htbp]
%   \centerline{\includegraphics[width=\linewidth,height=0.4\textheight]{figures/NRT_PL.png}}
%   \caption{Enhanced NRT}
%   \label{fig}
% \end{figure}

Voice data is a treasure trove of information, revealing a diverse range of speaker characteristics. These can include demographic details such as geographical origin, race, or education level; medical traits like the use of medications, neurological, or genetic disorders; physical attributes including gender, height, weight, and facial structure; physiological traits such as age and blood pressure; and much more \cite{singh2019profiling}. Given the depth and diversity of insights voice data can offer, the ability to model these vocal attributes accurately is becoming increasingly important. One widely explored task in this domain is age estimation from voice, which involves predicting a person's age based on their speech. Age estimation is formulated as a regression problem where the goal is to predict a real-valued number within a typical range, such as 10 to 80 years.

However, collecting age data for voice is challenging. It requires recording a person's voice and knowing their exact age at the time of recording. Consequently, age-labeled data is limited; as far as we know, the most trusted dataset for age estimation is the TIMIT dataset \cite{garofolo1993darpa}. The limited availability of labeled data with a wide range of age information presents a significant challenge for training complex models. Deep learning models, which excel at capturing non-linear relationships, require large amounts of data for effective training. On the other hand, simpler models like linear regressions require far fewer data points but often lack the flexibility to generalize well. Therefore, a reasonable strategy is to leverage the strengths of both approaches by learning to decompose the complex non-linear problem into multiple simpler linear functions—a concept known as piecewise linear modeling.


Piecewise linear problems involve approximating a function using multiple linear models, each applicable to a specific region or interval of the input space. This approach requires the joint optimization of partition boundaries and local linear models, a combinatorial problem that is difficult to optimize. Many existing methods simplify this problem by making assumptions about the data space, often leading to suboptimal solutions \cite{hawkins1976point}.

A promising technique for addressing this challenge is Regression-via-Classification (RvC) \cite{torgo1997regression, memon2019neural, zhao2021hierarchical}. RvC techniques use classifiers to find change points that discretize the output into predefined categories, each representing a specific range of the continuous outcome. 


Building upon this idea, we propose a new model called the Tessellated Linear Model. This model retains the simplicity of low-order functions, like linear functions, while achieving the capacity to approximate complex non-linear relationships akin to neural networks. The Tessellated Linear Model partitions the input space into convex sets that form a cover and models the function within each set using a linear model. Both the tessellation and the linear estimators within each region are optimized jointly for the overall prediction task.


We apply our model to a challenging voice biometric task—age prediction from voice—and demonstrate that it outperforms traditional neural models trained on TIMIT dataset. Our approach belongs to the RvC family and aims to learn an optimal piecewise linear predictor over linear tessellations of the input space.  We transform a complex combinatorial optimization problem into a more manageable learning problem by scanning optimal thresholds to partition the space based on the response variable. We then use binary classifiers to tessellate the space according to these chosen thresholds.



The key contributions of this paper are:

\begin{enumerate}
    \item A simplified model for piecewise linear functions that uses linear regression and logistic regression classifiers to tessellate the space and fit a linear model in each segment.
    \item A comparison of different training and inference strategies.
    \item Evaluation on two regression tasks from voice data: age prediction and height prediction.
    % \item An evaluation benchmark for age prediction based on Queen Elizabeth II's recordings from 1953 to 2021.
\end{enumerate}

In the following sections, we formally describe the Tessellated Linear Model, present experimental results, and discuss the implications of this approach for regression problems in various domains.







% \begin{figure}[htbp]
%   \centerline{\includegraphics[width=\linewidth,height=0.4\textheight]{figures/NRT_PL.png}}
%   \caption{Enhanced NRT}
%   \label{fig}
% \end{figure}
